Adversarial Pre-Padding: Generating Evasive Network Traffic Against Transformer-Based Classifiers

To date, traffic obfuscation techniques have been widely adopted to protect network data privacy and security by obscuring the true patterns of traffic. Nevertheless, as the pre-trained models emerge, especially transformer-based classifiers, existing traffic obfuscation methods become increasingly vulnerable, as witnessed by current studies reporting the traffic classification accuracy up to 99\% or higher. To counter such high-performance transformer-based classification models, we in this paper propose a novel and effective \underline{adv}ersarial \underline{traffic}-generating approach (AdvTraffic\footnote{The code and data are available at: https://anonymous.4open.science/r/TrafficD-C461}). Our approach has two key innovations: (i) a pre-padding strategy is proposed to modify packets, which effectively overcomes the limitations of existing research against transformer-based models for network traffic classification; and (ii) a reinforcement learning model is employed to optimize network traffic perturbations, aiming to maximize adversarial effectiveness against transformer-based classification models. To the best of our knowledge, this is the first attempt to apply adversarial perturbation techniques to defend against transformer-based traffic classifiers. Furthermore, our method can be easily deployed into practical network environments. Finally, multi-faceted experiments are conducted across several real-world datasets, and the experimental results demonstrate that our proposed method can effectively undermine transformer-based classifiers, significantly reducing classification accuracy from 99\% to as low as 25.68\%.

==> sections/Preliminaries.tex <==
\section{Preliminaries} \label{sec:Preliminaries}

\subsection{Definitions}

A network flow can be represented as a tuple $NT=(P, D)$, where $P$ is a collection of sequential data packets, and $D$ is a vector of packet delays, i.e.,
% $D=[D_1, D_2, ..., D_m]$,
 % and $1 \textless 2 \textless \ldots \textless m$
\begin{center}
$P=[P_1, P_2, ..., P_n]$,  
\end{center}
where $1 \textless 2 \textless \ldots \textless n$. Here, $P_i$ denotes an individual network packet, and $n$ represents the total number of packets within the flow. A data packet is composed of a series of byte sequences. The number of bytes in the data packet is referred to as the length of the data packet and is denoted by $\|P_i\|$. 

% $D_i$ represents the delay time between two consecutive data packets.

\subsection{Problem Statement and Challenges}

\textbf{Our problem: Defeating pre-trained based traffic classification models.} Unlike existing adversarial approaches\cite{shenoi2023ipet}\cite{zolbayar2022generating}\cite{rahman2020mockingbird}\cite{wang2017walkie}\cite{ling2022towards}\cite{juarez2015wtf}, this study focuses solely on generating adversarial samples through padding to counteract pre-training methods that use traffic content as input. By altering the semantic structure of the data packets, this method deceives the deep learning classifier. Approaches that involve generating adversarial samples by inserting additional packets or delaying packet transmission are not considered in this study. Denote $\widetilde{P}=[\widetilde{P_1}, \widetilde{P_2}, ..., \widetilde{P_n}]$ as the adversarial version of network packets. $\widetilde{P_i}$ is represents the adversarial manipulation of original packet $P_i$. It should be noted that, since we only perform padding operations on the data packets, the lengths of both $P$ and $\widetilde{P}$ are both $n$. However, due to the padding, the overall data length of $\widetilde{P_i}$ becomes larger than that of $P_i$, i.e., $\|\widetilde{P_i}\| \geq \|P_i\|$

\textbf{Finding Adversarial Samples.} Let $f(\cdot)$ be a classifier function that takes an arbitrary packet $\mathbf{x}$ and outputs a label, i.e., $f(\mathbf{x})=y$, where $y \in \Phi$, and $\Phi$ represents the set of possible labels. An adversarial example is crafted to deceive the classifier into making an incorrect classification. The adversary’s goal is to create adversarial examples by introducing minimal perturbations to the input data, ensuring that the changes are as imperceptible or small as possible. This can be framed as the following optimization problem:

\begin{equation} \label {equation-00}
    \mathbf{x^*} = \mathbf{x} + argmin\{\mathbf{\delta}: f(\mathbf{x+\delta}) \ne f(\mathbf{x})\} = \mathbf{x} + \mathbf{\delta}_x
\end{equation}
where $\mathbf{\delta}_x$ is the perturbation added to $\mathbf{x}$, and $\| \mathbf{\delta}_x \|$ denotes the norm of the perturbation, representing the magnitude of change. The constraint $f(\mathbf{x+\delta}) \ne f(\mathbf{x})$ ensures that the perturbed input $\mathbf{x} + \mathbf{\delta}_x$ is misclassified by the classifier $f(\cdot)$.

The symbol $^\text{"}+^\text{"}$ in adversarial examples holds distinct meanings across different fields, adapting to the data's structure:

\begin{itemize}
	\item 
 \textbf{Image Adversarial Attacks}. Here, The symbol, $^\text{"}+^\text{"}$, implies adjusting pixel values, modifying the intensity or color of specific pixels in the original image.. 
	\item 
 \textbf{Natural Language Adversarial Attacks}. For text, The symbol represents modifications such as replacing, inserting, or deleting words in the original sentence.

        \item 
 \textbf{Network Traffic Adversarial Attacks}. In this study, due to the limitations in directly altering individual bytes (e.g., via gradients), we instead apply padding to generate adversarial samples. Thus, The symbol signifies appending additional byte sequences to the original traffic flow, achieving an adversarial effect without modifying the existing byte values.
 
\end{itemize}

This adaptation of $^\text{"}+^\text{"}$ for network traffic adversarial generation allows effective adversarial manipulation while preserving the integrity of the original packet content.

\textbf{Bandwidth overhead.}
Bandwidth overhead is calculated as the ratio of the added bytes for defense to the bytes in the original, undefended packet. This overhead reflects the additional data load incurred between the client and the proxy or between proxies due to the insertion of adversarial byte sequences intended to protect against classification by pre-trained models. The additional bytes introduced for adversarial purposes are confined to the network segments where the client communicates with a proxy or where traffic traverses intermediary proxies. The accessed server itself remains unaffected by the overhead because the proxy removes the adversarial byte sequences before forwarding the traffic to the server. This ensures that the traffic appears normal and parseable to the server, maintaining regular server-client functionality without extra load on the server. The server does not generate additional byte sequences since its primary role is to provide services to all users, and traffic obfuscation is not within its responsibilities.

\textbf{Does the perturbation magnitude need to be constrained?}
Unlike adversarial sample generation in computer vision or natural language processing, where modification amplitude constraints are essential, we do not impose such constraints on network traffic payloads. In computer vision and NLP, adversarial examples must satisfy $L_1$, $L_2$ or $L_\infty$  norm bounds to ensure the original semantics of the image or text remain intact from a human perspective. 

For network traffic, modification amplitude refers to the number of bytes added or modified relative to the original byte sequence in the packet. As long as the payload is delivered intact and the sender and receiver can interpret the message identically, the semantic integrity of the communication remains unchanged, and normal functionality is maintained.. Consequently, minimizing modification amplitude is not a strict constraint in our problem, and fluctuations in single-byte values are acceptable. However, to prevent network performance degradation due to excessive traffic, it is still desirable to minimize the modification amplitude of network traffic—resulting in a smaller defense bandwidth overhead, which is preferable.

\textbf{Adversarial Training.} Recent studies demonstrate that adversarial training can enhance model robustness by incorporating adversarial examples into the training data\cite{qiao2023resisting}\cite{singh2024revisiting}\cite{madry2018towards}\cite{tramèr2018ensemble}. This approach trains models to recognize and classify adversarial examples, thereby improving classification accuracy. However, a notable limitation is that adversarial training may not generalize well to novel adversarial examples. In the networking domain, however, classifiers gain a unique advantage by anticipating adversarial examples, as attackers can intercept traffic at various network devices or links. For this reason, adversarial training remains a key focus in this research.




\textbf{Challenges.} Implementing traffic obfuscation technology presents several challenges. First, it is necessary to develop strategies for adding byte sequences that can effectively counter pre-trained traffic classification methods. Second, efficient methods are needed to insert the minimal number of byte sequences required to create effective adversarial samples while avoiding high bandwidth overhead that could interfere with normal communication. Finally, the defense must be resilient against adversaries aware of the obfuscation method; that is, the traffic obfuscation must withstand attempts to bypass it. Specifically, if an attacker intercepts traffic protected by a particular defense, they may retrain their classification model to overcome the obfuscation, necessitating a robust defense.

==> sections/ethic.tex <==
\section{Ethics Considerations}\label{sec:ethic}
First, the experimental data used in this study comprises two parts: publicly available data and data collected in a controlled environment. All data collection processes adhered to relevant laws and regulations, ensuring that sensitive information was anonymized during data processing to prevent privacy or ethical violations. Furthermore, the published code and datasets will exclude any sensitive user information, thereby safeguarding user privacy.


Second, although no real users actively attempt to evade censorship in this study, the proposed algorithm may involve interactions with censorship mechanisms, which could be considered illegal in restricted regions and potentially pose risks to operators. However, due to the black-box nature of censorship systems, such interaction is often the only feasible approach to evaluate the algorithm's effectiveness. This methodology is consistent with previous studies\cite{2019Geneva,2021Your}.

Finally, the model proposed in this paper aims to enhance privacy protection and security defense capabilities for network traffic during communication, with no intention to harm individuals or facilities.

==> sections/openscience.tex <==
\section{Open Science}\label{sec:Open}

This research adheres strictly to the conference's open science policy. Upon acceptance, the source code for this study will be made publicly available. Furthermore, as this research introduces a novel dataset, the dataset will also be released in compliance with ethical guidelines, ensuring no breach of user privacy. This initiative aims to facilitate experimental evaluation and further research by the academic community.


